On Infinite-horizon System Level Synthesis Problems

System level synthesis is a promising approach that formulates structured optimal controller synthesis problems as convex problems. This work solves the distributed linear-quadratic regulator problem under communication constraints directly in infinite-dimensional space, without the finite-impulse response relaxation common in related work. Our method can also be used to construct optimal distributed Kalman filters with limited information exchange. We combine the distributed Kalman filter with state-feedback control to perform localized LQG control with communication constraints. We provide agent-level implementation details for the resulting output-feedback state-space controller.

==> tex_files/01_introduction.tex <==
\section{INTRODUCTION}

In recent years, control design for networked dynamical systems has seen tremendous interest and progress.
An important problems is to impose structures on the controllers, such as sparsity for distributed or localized control \cite{han2003lmi,lessard2012optimal, wang2014localized}, and communication delay constraints \cite{wang2014localized, feyzmahdavian2012optimal}. Such control design problems are challenging due to the non-convex nature of the problem \cite{rotkowitz2005characterization}. 

Lately, many works have focused on novel controller parameterization that admits convex formulation \cite{wang2019system, furieri2019input, sabuau2021network}, with System Level Synthesis (SLS) emerging as a promising and unified framework for structured controller synthesis \cite{anderson2019system}. A vital feature of the SLS framework is that both the synthesis and the implementation of the structured controller can be done \textit{locally}, thus scaling favorably with the number of subsystems in a network. 
Most of the work in SLS literature focuses on the state-feedback case. Therefore, the state-feedback theory of SLS has been studied extensively both in terms of the controller parameterization \cite{matni2017scalable, ho2020system, yu2020achieving} and controller implementation \cite{li2020separating, yu2021localized}. However, similar aspects of the output-feedback case remain elusive. Since \cite{wang2016localized} first laid out the output-feedback SLS framework, \cite{boczar2018finite} made progress towards robustness and
\cite{conger2021output} proposed a computational speedup.


% control design is of great importance due to its relevance in practice where the states of a system can not be directly observed \cite{sadabadi2016static}. 


However current all SLS-based methods require both the parameterization and implementation to have finite impulse responses (FIR), with the exception of \cite{yu2021localized}.
% Synthesizing an FIR closed-loop requires the open-loop system to be observable and controllable.
% Therefore, lifting the FIR constraint will render SLS applicable to detectable and stabilizable systems.
This is because
{optimal controller synthesis, despite the choice of convex reparameterization, is an infinite-dimensional non-convex optimization problem over dynamical systems. 
% SLS and other versions of Youla parameterization make costs and constraints that are convex in the closed-loop convex in the optimization variable. While convexity gives us hope, solving infinite-dimensional problems can be daunting. 
The current method of choice to relax the problem into a tractable \emph{finite-dimensional} optimization problem is to restrict the optimization variable to having a finite impulse response. Such relaxation technique is required for many other parameterizations \cite{zheng2022system}. However, as previous work almost exclusively uses FIR approximations, we risk blindsiding ourselves into thinking that it is a requirement for SLS rather than a convenient relaxation to use off-the-shelf optimization software.} 
Moreover, synthesizing an FIR closed-loop requires the open-loop system to be observable and controllable. 
Therefore, lifting the FIR constraint will render SLS applicable to detectable and stabilizable systems. 
An exception is \cite{yu2021localized}, where the authors showed that the infinite-horizon state-feedback SLS problem has natural connections to the Riccati solution for LQR. It is a natural next step to investigate the correspondence between infinite-horizon output-feedback SLS and the LQG theory \cite{wonham1968separation}. Such investigation can expose the structure of output-feedback SLS, analogous to the estimator-controller separation structure of classical centralized LQG control. In the same work, \cite{yu2021localized} proposes a novel state-space realization of the SLS controllers, which circumvent the growing memory requirement for FIR SLS controllers, it is plausible that such memory reduction exists for infinite-horizon output-feedback SLS controllers, which will result in more efficient controller implementation. 



\textbf{Contribution. }
This paper investigates the infinite-horizon output-feedback SLS problem that corresponds to a class of LQG problems with structural constraints expressable as convex sparsity constraints under the SLS parameterization. Our contribution is four-fold.
\begin{itemize}
     \item We provide the first solution to this infinite-horizon problem, lifting previous restrictions on the applicability of output-feedback SLS theory due to the finite-horizon approximation. Our solution leverages an analogous separation principle for SLS parameterization. In particular, we solve an infinite-horizon structured state-feedback SLS problem and an infinite-horizon structured Kalman-filter SLS problem separately and construct a feasible solution to the output-feedback structured SLS problem from the two solutions. A key advantage of our solution is the ability to compute the parameters of each subsystem locally in one swoop using \textit{local}in formation without the iterations or communications among subsystems required by previous methods.\footnote{Output-feedback SLS problems, structured or not, require alternating direction method of multipliers (ADMM)-style iterative optimization method for local computation [cite]. See [cite] for more details.} 
    \item We generalize a result on the infinite-horizon state-feedback SLS solution \cite{yu2021localized} that we use to construct output-feedback controllers that handle communication delays among subsystems.
    \item Our controller has a lower memory requirement than existing FIR-based SLS controllers.  
    \item  We study the suboptimality of our proposed method numerically. \jnote{add numerics result here.}   %The simulation findings corroborate with the theoretical results where our solution achieves optimality for unstructured LQG problems while we... 
\end{itemize}


\textbf{Related Work. }
There is a large and growing body of work on the topics of distributed control. Here we briefly review the literature most relevant to this work.

\textit{Distributed Output-feedback Control}: Since \cite{rotkowitz2005characterization}, optimal distributed control problems have been largely studied through the lens of convexification \cite{lessard2012optimal, fazelnia2016convex, lamperski2013output, tanaka2014optimal} by restricting to the class of structural constraints with Quadratic Invariance (QI) property. Going beyond QI, recent advances in the field have primarily focused on parameterization of stabilizing controllers that admits broader classes of nonconvex structural constraints on the controller as convex constraints on the parameters \cite{wang2019system, furieri2019input}, with \cite{zheng2020equivalence} and \cite{tseng2021realization} clarifying the connections among various approaches to parameterization. Recently, \cite{sabuau2021network} adopts Youla parameterization and proposes a new framework for distributed output-feedback controller implementation without any internal states exchanges. This work improves the scalability of controller implementation and adopts a centralized synthesis scheme. Our work contributes to this line of research by proposing a state-space output-feedback controller that handles structural constraints not necessarily QI. 

\textit{System Level Synthesis:} The SLS framework has found useful application in various areas of control theory where most work focused on state-feedback control design, see \cite{anderson2019system} and \cite{shuang2020frontiers} for some references. The output-feedback case received relatively less attention. Following the distributed synthesis and implementation of SLS controller given in \cite{wang2016localized} with FIR approximation, robustness issue \cite{boczar2018finite} and computational speedup \cite{conger2021output} of the output-feedback FIR SLS control design have been investigated. Our work leverages the infinite-horizon state-feedback SLS solution in \cite{yu2021localized} and provide the first infinite-horizon solution to the output-feedback SLS problem. 
% In particular, our approach draws connections between output-feedback SLS and the separation principle of classical LQG control \cite{wonham1968separation}.


\textbf{Notation. }
% We denote real-valued vectors $x \in \R^n$ and matrices $M \in \R^{n \times m}$ using lower and upper case respectively. 
Bold font $\mathbf x$ and $\mathbf G$ denotes signals $\mathbf{x} = \{x(t) \}_{t = 0}^\infty$ with $x(t) \in \R^n$and causal transfer matrices $\mathbf{G}(z) = \sum_{i = 0}^\infty z^{-i}G[i]$ with kernels $G[i]\in \R^{m \times n}$. The $j^\text{th}$ standard basis vector is denoted as $e_j$. For a matrix $A$, $A(i, j)$ refers to the $(i, j)^\text{th}$ element, $A(i, :)$ to the $i^\text{th}$ row and $A(:, j)$ to the $j^\text{th}$ column. Nonnegative integers are $\mathbb{N}_{+}$. 
% For two binary matrices $S_1, S_2 \in \{0, 1\}^{m \times n}$, the operation $S_1 \cup S_2$ performs an element-wise OR operation. Given a matrix $A$, $\Sp(A)$ denotes the support of $A$ and we say that $\Sp(A) \subseteq S_1$ if $\Sp(A) \cup S_1 = S_1$. For a natural number $N$, we abbreviate the set $\{1, 2, \ldots, N\}$ as $[N]$.

% \onote{I think we should get rid of $S_1 \cup S_2$, $\Sp(A)$ as they won't be used much. We can just explain what they mean when we use them.} \jnote{But the definition of $A \in S_1$ requires we first specify what $\Sp(A) \cup S_1 $ means. Unless we want to explain $\Sp(A) \cup S_1$ in words.}
% \onote{If we only use it once in the article, there's no need to include it in the notation section... I think it's better to explain it where it's used in such cases.}

==> tex_files/02_body.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=.95\textwidth]{figures/OF_certainty.pdf}
    \caption{Caption}
    \label{fig:observer_feedback}
\end{figure*}




\section{Preliminaries}
\label{sec:prelim}

In this paper, we consider the following dynamical system
\begin{equation}
    \label{eq:dynamics}
    \begin{aligned}
        x(t+1) & = Ax(t) + Bu(t) + w(t) \\
        y(t) & = Cx(t) + v(t),
    \end{aligned}
\end{equation}
where $w(t)\sim \mathcal{N}(0,W)$, and $v(t)\sim \mathcal{N}(0,V)$ are respectively state and measurement noise independently and identically drawn at each time from the zero-mean Gaussian distributions, where they are uncorrelated. Here $W$ and $V$ are symmetrical positive definite matrices. The general control design objective is to synthesize a linear controller $\mathbf{K}$ such control action computed as $\mathbf{u} = \mathbf{Ky}$ stabilizes the closed-loop system. 

\subsection{System Level Synthesis}
% \onote{Write the SLPs for SF, FC and OF. Show how to construct a feasible solution starting from SF and FC. Show implementation with Jing's block diagram. Cite the corresponding article.}

The SLS theory approaches the output-feedback control design problem descibed above by characterizing all achievable closed-loop mappings (CLMs) from $\mathbf{w},\mathbf{v}$ to $\mathbf{x}$, $\mathbf{u}$ under an internally stabilizing controller $\mathbf{K}$. Then, using any achievable CLMs, SLS provides an implementation of the controller $\mathbf{K}$ that realizes the prescribed CLMs. This is made precise in the following result.

\begin{theorem}[\cite{anderson2019system}]
\label{thm:sls}
Any linear CLMs $\bPhi_{xx}$, $\bPhi_{xy}$, $\bPhi_{ux}$, $\bPhi_{uy} \in \frac{1}{z} \R\mathcal{H}_\infty$ can be achieved by a linear internally stabilizing controller $\mathbf{K}$ if and only if
\begin{subequations}
\label{eq:output-feasibility}
\begin{align}
    \bmat{zI - A & -B_2} \PHI & = \bmat{I & 0} \label{eq:feasibility_x}\\
    \PHI \bmat{zI - A \\ -C_2} & = \bmat{I \\ 0}, \label{eq:feasibility_u}
\end{align}
\end{subequations}
where $\bPhi_{xx}$, $\bPhi_{xy}$, $\bPhi_{ux}$, $\bPhi_{uy}$ maps $\mathbf{w},\mathbf{v}$ to $\mathbf{x}$, $\mathbf{u}$ under a controller $\mathbf{K}$, i.e.,$\xu = \PHI \wv $. 
In particular, $\mathbf{K}$ can be implemented as the following, which is illustrated in Figure \ref{fig:sls_of}:
% The controller realization in \ref{fig:sls_of_structure} results in an internally stable closed-loop system.
% The control signal \ref{fig:sls_of_structure} is computed as
\begin{equation}
    \label{eq:of-controller}
    \begin{aligned}
        z\bbeta & = \hbPhi_{xx}\bbeta + \hbPhi_{xy}\by \\
        \bu & = \hbPhi_{ux}\bbeta + \bPhi_{uy}\by,
    \end{aligned}
\end{equation}
where $\hbPhi_{xx} = z(I - z\bPhi_{xx})$, $\hbPhi_{ux} = z\bPhi_{ux}$, $\hbPhi_{xy} = -z\bPhi_{xy}$.
\end{theorem}
 Further, it was shown in \cite{wang2019system} that \eqref{eq:output-feasibility} is equivalent to stabilizability and detectability of the system \eqref{eq:dynamics}. Therefore, \eqref{eq:of-controller} parameterizes all internally stabilizing linear controller $\mathbf{K}$ for \eqref{eq:dynamics}. 

A special case of Theorem \ref{thm:sls} is when the controller is \emph{state-feedback}, i.e., $\mathbf{u} = \mathbf{K}\mathbf{x}$. In this scenario, SLS parameterizes all stabilizing state-feedback controller with CLMs that maps $\mathbf{w}$ to $\mathbf{x}$ and $\mathbf{u}$ only.   



\begin{figure}
    \centering
    \input{figures/output-structure}
    \caption{Stolen without permission (yet). $\hbPhi_{xx} = z(I - z\bPhi_{xx})$, $\hbPhi_{ux} = z\bPhi_{ux}$, $\hbPhi_{xy} = -z\bPhi_{xy}$}
    \label{fig:sls_of}
\end{figure}


\subsection{System-level Constraints (SLCs)}
For large-scale networked systems, it is common to impose structural constraints such as localization requirement and communication delay on $\mathbf{K}$. A large class of such structural constraints can be characterized as convex constraints on CLMs. This is called the system-level constraints (SLCs) \cite{wang2019system}. Examples of SLCs include constraints on the Youla parameter, QI subspace constraints on $\mathbf{K}$, and FIR constraints on the closed-loop responses to noises. 

In this paper, we consider the family of SLCs that can be represented as sparsity constraints on the CLMs. We denote any such sparsity constraints as $\s := \{S[k]\}_{k=1}^\infty$ where each $S[k]\in \{0,1\}^{n \times n}$ are binary matrices specifying the sparsity of the kernels of CLMs. An important example of this family of SLCs are the \textit{localization SLCs} that specifies how disturbances at each subsystem must be localized to a neighborhood \cite{yu2021localized}.
\begin{definition}[Localization SLCs]
An SLC $\s := \{S[k]\}_{k=1}^\infty$ is called the localization SLC if $S[k]$ for all $k$ are the same binary matrices.
\end{definition}
Another important sparsity constraints are \textit{communication delay SLCs}. We use $\text{Sp}(\cdot)$ to denote the support of a matrix.
\begin{definition}[Communication delay SLCs]
For a fixed integer $d$ and sparsity pattern of the dynamics $\mathbb{A} := \text{Sp}\left(A \right)$, a communication delay SLC is such that $S[k] = \text{Sp}\left(\mathbb{A}^k\right)$ for $k\leq d$ and $S[k] = \text{Sp}\left(\mathbb{A}^k\right)$ for all $k \geq d$.
\end{definition}
This is sometimes called the $(A,d)$-sparsity \cite{wang2014localized}. We say $\bPhi_{xx} \in \s$ if $\Phi_{xx}[k]$ has the same sparsity pattern as $S[k]$ for all $k \in \mathbb{N}_{+}$. 


\subsection{The Structured Output-feedback SLS Problem}
We now state the output-feedback SLS problem with general sparsity SLCs that this paper aims to investigate,
\begin{equation}
\begin{array}{rl}
 \underset{\bPhi}{\text{min}}  &  \norm{\begin{bmatrix}Q^{1/2} & 0 \\ 0 & R^{1/2}\end{bmatrix} \PHI \begin{bmatrix}W^{1/2} & 0 \\ 0 & V^{1/2}\end{bmatrix}}_{\mathcal{H}_2} \tag{OF-SLS}\\
\text{s.t.} &  \text{constraints \eqref{eq:output-feasibility}}\\
& \bPhi_{xx}, \bPhi_{ux},\bPhi_{xy},\bPhi_{uy} \in  \s.
\end{array}
\label{eq:of-original}
\end{equation}
where we used $\bPhi$ to collectively refer to the tuple $\left(\bPhi_{xx}, \bPhi_{ux},\bPhi_{xy},\bPhi_{uy}\right)$ to reduce notation. The objective function in \eqref{eq:of-original} corresponds to the classical LQG problem with cost $\mathbb{E} \sum_{t}^\infty {x(t)}^{\top} Q x(t) + {u(t)}^{\top} R u(t) $ under uncorrelated state and measurement noise. Therefore, \eqref{eq:of-original} can be viewed as an LQG problem with the class of structural constraints expressable as static sparsity SLCs.

\textbf{Infinite Horizon vs FIR.} We note that \eqref{eq:of-original} is an infinite-horizon problem in $\bPhi$. Therefore, previous work resorts to finite-impulse-response (FIR) approximation, where an additional FIR requirement is imposed on $\bPhi$. However, \eqref{eq:of-original} with FIR constraint is not feasible for general stabilizable and detectable systems \cite{anderson2019system}, thus significantly restricts the applicability of output-feedback SLS for structured LQG problems. Moreover, the number of optimization variables grows linearly with the FIR horizon length, which can become prohibitive for large-scale systems. 

\textbf{Distributed Iterative Computation.} For scalability, existing methods leverage the partial separability of \eqref{eq:of-original} and solve \textit{locally} the individual rows and columns of $\bPhi$ iteratively until convergence \cite{anderson2019system}.

\textbf{Memory-intensive Implementation.} When $\bPhi$ are constrained to be FIR filters of horizon $H$, existing controller implementation \eqref{eq:of-controller} keeps track of a history of the internal variables up to $H$ length. As mentioned above, such memory requirement scales linearly with $H$ and pose challenges to the scalability of \eqref{eq:of-controller} in large systems.
 

In what follows, we improve the three issues above by providing alternative approach that gives the first infinite-horizon CLM solution to \eqref{eq:of-original} without iteration (Section \ref{sec:solution}) by combining a structured state-feedback SLS solution and a structured state-observer SLS solution. We also propose a state-space controller that implements the infnite-horizon CLMs and provide new details of information exchange of the controller implementation (Section \ref{sec:controller}). Moreover, we generalize the previous infinite-horizon state-feedback SLS method to handle general delay sparsity constraints as opposed to only static localization sparsity constraints (Section \ref{sec:delay}). Finally, we use simulation to investigate the optimality gap between the proposed output-feedback SLS solutions and the optimal solutions computed numerically (Section \ref{sec:simulation}).



\section{A solution Inspired by Separation Principle}
\label{sec:solution}
In this section, we leverage the infinite-horizon state-feedback SLS solution (Theorem \ref{thm:inf-sf-sls}) to construct a feasible infinite-horizon solution to \eqref{eq:of-original} via an analogous separation principle for SLS parameterization (Theorem \ref{thm:observer_feedback}). 


\subsection{Infinite-horizon State-feedback SLS}
For any state-feedback systems, e.g., \eqref{eq:dynamics} with $C = I$ and $v(t) \equiv 0$, we can synthesize the optimal structured state-feedback CLMs from $\mathbf{w}$ to $\mathbf{x}$ and $\mathbf{u}$, denoted as $\bPhi_{xw}$ and $\bPhi_{uw}$ respectively. 
The following result provides the solution to the structured state-feedback SLS problem, which we present in simplified form. For the full description, readers are referred to section IV in \cite{yu2021localized}.
% \jnote{How bad would it be if I just leave the details out? Dont really want to write out exactly what the transformed matrices are.. }
\begin{theorem}[\cite{yu2021localized}]
\label{thm:inf-sf-sls}
Fix localization SLCs $\s^L_x$ and $\s^L_u$, the infinite-horizon optimal solution $\bPhi_{xw}^\star$, $\bPhi_{uw}^\star$ to the following structured infinite-horizon state-feedback SLS problem:
\begin{align}
\label{eq:sf-sls}
& \underset{\bPhi_{xw},\bPhi_{uw} \in \frac{1}{z} \R\mathcal{H}_\infty}{\text{min}} 
& & \norm{\bmat{Q^{1/2} & 0 \\ 0 & R^{1/2}} \bmat{\bPhi_{xw} \\ \bPhi_{uw}}}_{\mathcal{H}_2}  \\
& \text{subject to}
& & \bmat{zI - A & -B}\bmat{\bPhi_{xw} \\ \bPhi_{uw}} = I \nonumber\\
&&& \bPhi_{xw} \in \s^L_x, \quad \bPhi_{uw} \in \s^L_u \nonumber
\end{align}

is given in a column-wise fashion by
\begin{align*}
  \bPhi_{xw}^\star(:,i) = \ssreal{A^{\text{SF}, i}}{e_i}{I}{0}  ,\quad  \bPhi_{uw}^\star(:,i) = \ssreal{A^{\text{SF}, i}}{e_i}{K^i}{0}   \, ,
\end{align*}
where $A^{\text{SF}}$, $K^i$ are the state space system matrices associated with the $i^{\text{th}}$ column of $\bPhi_{xw}^\star$ and $\bPhi_{uw}^\star$, which can be computed with discrete-time Riccati equation under transformation.
\end{theorem}
For fixed localization SLCs, we denote \eqref{eq:sf-sls} as $\SF{A,\,B,\,Q\,,R}$ and write the optimal state-feedback SLS solution as $\left(\bPhi_{xw}^\star, \bPhi_{uw}^\star \right)= \SF{A,\,B,\,Q\,,R}$. 

Theorem \ref{thm:inf-sf-sls} can be used to solve the dual problem of optimal structured Kalman filter design with localization SLCs for \eqref{eq:dynamics} \cite{wang2015localized}. In particular, the optimal structured infinite-horizon CLMs that map $\mathbf{w}$ and $\mathbf{v}$ to state estimation error $\mathbf{e}$ under a linear observer $\mathbf{L}$ with respect to the mean estimation error is given by  
$\left(\bPhi_{ew}^\star, \bPhi_{ev}^\star \right)= \left( \SF{A^{\top},\,C^{\top},\,W\,,V}\right)^\top$, i.e., the solution to
\begin{align}
\label{eq:kf-sls}
& \underset{\bPhi_{ew},\bPhi_{ev} \in \frac{1}{z} \R\mathcal{H}_\infty}{\text{min}} 
& & \norm{\bmat{W^{1/2} & 0 \\ 0 & V^{1/2}} \bmat{\bPhi_{ew}^\top \\ \bPhi_{ev}^\top}}_{\mathcal{H}_2}  \\
& \text{subject to}
& & \bmat{\bPhi_{ew} & \bPhi_{ev}} \bmat{zI - A \\ -C}= I \nonumber\\
&&& \bPhi_{ew} \in \s^L_x, \quad \bPhi_{ev} \in \s^L_u. \nonumber
\end{align}
Readers are referred to \cite{wang2015localized} for more details.

\subsection{A feasible solution to \eqref{eq:of-original}}
It is well known that for linear systems, a stabilizing output-feedback controller for centralized LQG problems can be constructed from a stabilizing state-feedback controller and a stable state observer. In \cite{wang2019system}, the authors pointed out that a similar property holds for CLMs from state-feedback and kalman-filter SLS problem. 

\begin{theorem}[\cite{anderson2019system}]
\label{thm:observer_feedback}
Assume there exist stable and strictly causal transfer matrices $\Phisf = (\Phisf_{xw},\Phisf_{uw})$ and $\Phifc = (\Phifc_{ew}, \Phifc_{ev})$ satisfying

\begin{align}
    \bmat{zI - A & -B}\bmat{\Phisf_{xw} \\ \Phisf_{uw}} & = I, \\
    \bmat{\Phifc_{ew} & \Phifc_{ev}}\bmat{zI - A \\ -C} & = I.
\end{align}
The transfer functions
\begin{equation}\label{eq:certainty_equivalence}
\begin{aligned}
    \bPhi_{xx} & = \Phisf_{xw} + \Phifc_{ew} - \Phisf_{xw}(zI - A)\Phifc_{ew} \\
    \bPhi_{ux} & = \Phisf_{uw} - \Phisf_{uw}(zI - A)\Phifc_{ew}\\
    \bPhi_{xy} & = \Phifc_{ev} - \Phisf_{xw}(zI - A)\Phifc_{ev} \\
    \bPhi_{uy} & = - \Phisf_{uw}(zI - A)\Phifc_{ev}
\end{aligned}
\end{equation}
are strictly causal and satisfy \eqref{eq:output-feasibility}.
\end{theorem}

With Theorem \ref{thm:observer_feedback}, we can construct a \textit{feasible} solution with the solutions to $\SF{A,\,B,\,Q\,,R}$ and $\SF{A^{\top},\,C^{\top},\,W\,,V}$ via Theorem \ref{thm:inf-sf-sls}.

We point out that the infinite-horizon state-feedback SLS solutions given in Theorem \ref{thm:inf-sf-sls} can only handle static localization SLCs. This means that each local controller assumes instantaneous information exchanges among all other subsystems in a localization neighborhood. Such communication pattern can be unrealistic in some cases. In section \ref{sec:delay}, we address this problem by generalizing Theorem \ref{thm:inf-sf-sls} to accommodate communication delay SLCs. Consequently, the distributed output-feedback controller can stabilize the closed loop using delayed information from other subsystems in a localization neighborhood. 




\section{Local Controller implementation}
\label{sec:controller}


This section explains how to implement the controller in Fig.~\ref{fig:observer_feedback} locally and describes the communication between nodes. 
For each time step $t$, each node $i$ observes the local output, communicates with its neighbors and computes internal signals.
The entire procedure is summarized in Algorithm~\ref{alg:full}, which consists of four distinct stages where communication between neighbors must happen before the internal state $\bbeta_i$ is updated and the control signal $u_i(t)$ is applied.
Between each communication stage, the node must compute internal signals and simulate the local components of the dynamical systems in \ref{eq:certainty_equivalence} one step.
Subroutines~\ref{sub:1}--\ref{sub:4} describe these computations in detail.

\begin{algorithm}
\caption{Localized computation of controller signals}\label{alg:full}
\begin{algorithmic}
\For{Each node $i = 1, \ldots, N$}
    \State Initialize $\tPhisf_{xx, \alpha}(:, i)$, $\tPhisf_{xx, \zeta}(:, i)$, $\tPhifc_{xx}(:, i)$, $\tPhifc_{xy}(:, i)$
    \State $\beta_i(0) \gets 0$
    \State $w_i(t) \gets 0$
    \State $v_i(t) \gets 0$
\EndFor
\For{$t = 0, 1,  \ldots$}
\For{Each node $i = \{1, \ldots, N\}$} \Comment{parallel}
    \State Observe $y_i(t)$
    \State Receive $\beta_j(t)$ and $y_j(t)$ from $j \in \Nin^d(i)$
    \State subroutine1()
    \State Receive $\widehat w_j(t)$ and $\widehat v_j(t)$ from $j \in \Nin^A(i)$
    \State subroutine2()
    \State Receive $\widehat \alpha^{(\Nout^d(j))}(t+1)$, $\widehat \zeta^{(\Nout^d(j))}(t+1)$, \\$\widehat \gamma^{(\Nout^d(j))}(t+1)$ and $\widehat \theta^{(\Nout^d(j))}(t)$ from $j \in \Nin^d(i)$.
    \State subroutine3()
    \State Receive $\alpha_j(t + 1)$ and $\gamma_j(t + 1)$ from $j\in \Nin^A(i)$
    \State subroutine4()
    \State Apply $u_i(t)$
\EndFor
\EndFor
\end{algorithmic}
\end{algorithm}

The initialization of Algorithm~\ref{alg:full} requires the local components of \eqref{eq:certainty_equivalence}, from \onote{where?}: 
\begin{align*}
\renewcommand\arraystretch{1.4}
    \tPhisf_{xx}(:, i) & = \ssreal{A_{xx}^{\text{SF}, i}}{e_i}{I}{0}, &
    \tPhisf_{ux}(:, i) & = K_i\tPhisf_{xx}(:, i)\\
    \tPhifc_{xx}(i, :) & = \ssreal{A_{xx}^{\text{SF}, i}}{I}{e_i^\tran}{0},
    & \tPhifc_{xx}(i, :) & = \tPhifc_{xx}(i, :)L_i.
\end{align*}
From \eqref{eq:certainty_equivalence} and \eqref{eq:greek_letters}, we see that some, but not all, local subsystems can share states --- simplifying computation and reducing memory requirements.
We will however, require two instantiations of $\tPhisf_{xx}(:, i)$ to compute $\balpha$ and $\bzeta$ which we call $\tPhisf_{xx, \alpha}(:, i)$ and $\tPhisf_{xx, \zeta}(:, i)$ respectively.
Control-signal computation at the node $i$ begins by receiving the measurements from neighbors at most $d$ steps away, and computing the $i$th element of $\hat v(t + 1)$ and $\hat w(t + 1)$.
This stage is outlined in Subroutine~\ref{sub:1}, and illustrated in Fig.~\ref{fig:sub1}. 

\begin{Subroutine}
\caption{Compute $\widehat w_i(t + 1)$ and $\widehat v_i(t + 1)$}\label{sub:1}
\begin{algorithmic}
    \State Receive $\beta_j(t)$ and $y_j(t)$ from $j \in \Nin^d(i)$
    \State $\beta_{[\Nin^d(i)]}(t) \gets \text{vec}(\beta_{j_1}(t), \ldots, \beta_{j_m}(t)$
    \State $y_{[\Nin^d(i)]}(t) \gets \text{vec}(y_{j_1}(t), \ldots, \widehat y_{j_m}(t)$
    \State $\widehat w_i(t + 1) \gets \text{step}(z\tPhifc_{xx}(i, :), \beta_{[\Nin^d(i)]}(t))$
    \State $\widehat v_i(t + 1) \gets \text{step}(z\tPhifc_{xy}(i, :), y_{[\Nin^d(i)]}(t))$
\end{algorithmic}
\end{Subroutine}

\begin{figure}
    \centering
    \input{figures/phi_y}
    \caption{Illustration of subroutine 1. The computation of $\widehat w$ is similar.}
        \label{fig:sub1}
\end{figure}

In the second stage, the node receives $\widehat v_j(t)$ and $\widehat w_j(t)$ from its closest neighbors and computes the outgoing components of \eqref{eq:greek_letters}.
The computations are outlined in Subroutine~\ref{sub:2} and illustrated in \ref{fig:sub2}.

\begin{figure*}
    \centering
    \input{figures/subroutine_2}
    \caption{Illustration of subroutine 2.}
    \label{fig:sub2}
\end{figure*}

\begin{Subroutine}
\caption{Compute the outgoing components of \eqref{eq:greek_letters}}\label{sub:2}
\begin{algorithmic}
    \State $\widehat w_{[\Nin^A(i)]}(t) \gets \text{vec}(\widehat w_{j_1}(t), \ldots, \widehat w_{j_m}(t))$
    \State $\widehat v_{[\Nin^A(i)]}(t) \gets \text{vec}(\widehat v_{j_1}(t), \ldots, \widehat v_{j_m}(t)) $  \vspace{.2em}
    \State $\widetilde w_i(t) = \beta_i(t) +A\widehat w_{[\Nin^A(i)]}(t) - \widehat w_i(t+1)$ 
    \State $\widetilde v_i(t) = A\widehat v_{[\Nin^A(i)]}(t) - \widehat v_i(t+1)$
    \State $\widehat \alpha^{(\Nout^d(j))}(t+1)  \gets \text{step}(\tPhisf_{xx, \alpha}(:, i), e_i\widetilde w_i(t))$
    \State $\widehat \zeta^{(\Nout^d(j))}(t+1)  \gets \text{step}(\tPhisf_{xx, \zeta}(:, i), e_i\widetilde v_i(t))$ \vspace{.1em}
    \State $\widehat \gamma^{(\Nout^d(j))}(t + 1) \gets K_i\widehat \alpha^{(\Nout^d(j))}(t+1)$
    \State $\widehat \theta^{(\Nout^d(j))}(t) \gets K_i\widehat \zeta^{(\Nout^d(j))}(t)$
\end{algorithmic}
\end{Subroutine}

In the third stage, the node receives the components pertaining to its element of the signals in \eqref{eq:certainty_equivalence} from other nodes a distance at most $d$ steps away and sums them to compute the $i$th element of each esignal in $\eqref{eq:greek_letters}$.
This step is described in Subroutine~\ref{sub:3} and illustrated in Fig.~\ref{fig:sub3}.

\begin{figure}
    \centering
    \input{figures/subroutine_3}
    \caption{Illustration of subroutine 3.}
    \label{fig:sub3}
\end{figure}

\begin{Subroutine}
\caption{Compute the local elements of \eqref{eq:greek_letters}}\label{sub:3}
\begin{algorithmic}
    \State $\alpha_i(t+1) \gets \widehat w_i(t+1) + \sum_j\widehat\alpha^{(\Nout(j))}_i(t+1)$
    \State $\gamma_i(t + 1) \gets \sum_j \widehat\gamma^{(\Nout(j))}_i(t+1)$
    \State $\zeta_i(t + 1) \gets \widehat v_i(t+1) + \sum_j \widehat\zeta^{(\Nout(j))}_i(t + 1)$
    \State $\theta_i(t) \gets \sum_j\widehat\theta^{(\Nout(j))}_i(t)$
\end{algorithmic}
\end{Subroutine}

In the final stage the node receives $\alpha_j(t + 1)$ and $\gamma_j(t + 1)$ from its closest neighbors and computes $\beta_i(t + 1)$ and $u_i(t)$.

\begin{Subroutine}
\caption{Compute $u_i(t)$ and $\beta_i(t + 1)$}\label{sub:4}
\begin{algorithmic}
    \State $\alpha_{[\Nin^A(i)]}(t + 1) \gets \text{vec}(\alpha_{j_1}(t + 1), \ldots, \widehat \alpha_{j_m}(t + 1)$
    \State $\gamma_{[\Nin^A(i)]}(t + 1) \gets \text{vec}(\gamma_{j_1}(t + 1), \ldots, \widehat \gamma_{j_m}(t + 1)$ \vspace{-.75em}
    \begin{multline*}
        \beta_i(t + 1) \gets -A(i, :)\alpha_{[\Nin^A(i)]}(t + 1)\\ - B(i, :)\gamma_{[\Nin^A(i)]}(t + 1) - \zeta_i(t + 1)
    \end{multline*}% 
    \vspace{-1.5em}
    \State $u_i(t) \gets \gamma_i(t + 1) + \theta_i(t)$
\end{algorithmic}
\end{Subroutine}

We conclude with the observation that the node has now received information from nodes at most $2d + 2$ steps away.

\subsection{Internal stability}


\section{Generalization for Communication Delay}
\label{sec:delay}
The infinite-horizon state-feedback method \cite{yu2021localized} used to construct output-feedback SLS CLMs can only handle static localization SLCs, excluding communication delay SLCs. In this section, we derive the optimal infinite-horizon state-feedback SLS CLMs under communication delay SLCs. Our solution generalizes previous methods to a broader class of SLCs, and allows the subsequent output-feedback solutions to handle communication delays. 

\onote{New stuff goes here. Use aligned rather than align.}
\begin{align}
\label{eq:sf-sls_extended}
& \underset{\bPhi_{xw},\bPhi_{uw} \in \frac{1}{z} \R\mathcal{H}_\infty}{\text{min}} 
& & \norm{\bmat{Q^{1/2} & 0 \\ 0 & R^{1/2}} \bmat{\bPhi_{xw} \\ \bPhi_{uw}}}_{\mathcal{H}_2}  \\
& \text{subject to}
& & \bmat{zI - A & -B}\bmat{\bPhi_{xw} \\ \bPhi_{uw}} = I \nonumber\\
&&& \Phi_{xw}[k] \in \s_x[k], \quad \Phi_{uw}[k] \in \s_u[k] \nonumber
\end{align}
As \eqref{eq:sf-sls_extended} is column-wise separable, we will synthesize the closed-loop maps one column at a time.
From here on, everything will be as seen by the $i$th node, and we let $\bphixi := \bPhi_{xw}(:, i)$ and $\bphiui := \bPhi_{uw}(:, i)$ with the impulse responses $\phixi[k]$ and $\phiui[k]$ for $k = 0, 1, \ldots$.
Furthermore we let $s_x[k]$ and $s_u[k]$ denote the $i$th column of $S_x[k]$ and $S_u[k]$ respectively.
The corresponding problem to solve becomes
\begin{align}
    \underset{\bphixi, \bphiui}{\text{minimize:}} \quad & \sum_{k = 1}^\infty \phixi[k]^\tran Q\phixi[k] + \phiui[k]^\tran R\phiui[k] \nonumber \\
    \text{subject to:}\quad  & \phixi[k + 1] = A\phixi[k] + B\phiui[k]\label{eq:dynamics_extended}\\
    &\phixi[0] = 0, \quad \phixi[1] = e_i \nonumber \\
    &\phixi[k] \in s_x[k],\  \phiui[k] \in s_u[k].\label{eq:sparsity}
\end{align}
This new problem is a constrained linear quadratic optimal control problem, and would be a standard infinite-horizon LQR problem if it weren't for the sparsity constraints~\eqref{eq:sparsity}.
We will---with the help of some linear algebra---show how to transform this problem to a finite-horizon LQR problem with time-varying dynamics.
Let $n_x[k]$ be the number of nonzero elements in the $n$-dimensional vector $s_x[k]$ and $n_u[k]$ be the number of nonzero elements in $s_u[k]$.
Then there exists a surjective matrix $M_x[k]\in \R^{(n - n_x[k])\times n}$ and an injective matrix $M_u[k]\in \R^{n \times n_u[k]}$ such that \eqref{eq:sparsity} is equivalent to
\[
    M_x[k]\phixi[k] = 0,\quad \phiui[k] = M_u[k]w[k],
\]
where $w[k]\in \R^{n_u[k]}$ becomes our new optimization variable.
Since $\phixi[k + 1]$ is uniquely determined by the dynamics, $\phixi[k]$ and $\phiui[k]$, substitution into \eqref{eq:dynamics_extended} yields
\begin{equation}
    M_x[k + 1]A\phixi[k] + \underbrace{M_x[k + 1]BM_u[k]}_{F[k]}w[k] = 0.
    \label{eq:sparsity_knext}
\end{equation}
Equation \eqref{eq:sparsity_knext} has the solution
\begin{equation}
    w[k] = F[k]^\dagger M_x[k + 1]A\phixi[k] + N_F[k]v[k],
\end{equation}
where $N_F[k]\in \R^{n_u[k] \times n_v[k]}$ is an injective matrix such that $F[k] N_F[k] = 0$ and free $v[k]\in \R^{n_v[k]}$.
Substituting $\phiui[k] =M_u[k]w[k] $ into the optimal control problem we get the equivalent time-varying LQR problem
\begin{align*}
    \underset{v[k] \in \R^{m_v[k]}}{\text{minimize:}} \quad & \sum_{k = 1}^\infty \Big( \phixi[k]^\tran \tilde Q[k]\phixi[k] +  \\
    & \quad 2 v[k]^\tran \tilde Z\phixi[k] + v[k]^\tran \tilde R[k] v[k] \Big) \nonumber \\
    \text{subject to:}\quad  & \phixi[k + 1] = \tilde A_i\phixi[k] + \tilde B[k]v_k\\
    &\phixi[0] = 0, \quad \phixi[1] = e_i,
\end{align*}
where
\begin{equation}
    \begin{aligned}
    \tilde Q[k]  & = Q + \kappa[k]^\tran R \kappa[k] \\
    \tilde Z[k] & = N_F[k]^\tran M_u[k]^\tran R \kappa[k] \\
    \tilde R[k] & = (M_u[k]N_F[k])^\tran R[k] M_u[k]N_F[k]\\
    \kappa[k] & = M_u[k]F[k]^\dagger M_x[k + 1]A \\
    \tilde A[k] & = A - B\kappa[k] \\
    \tilde B[k] & = BM_u[k]N_F[k]
    \end{aligned}
\end{equation}
Finally we note that for $k \geq d + 1$, the localization patterns are constant implying that the dynamics of the transformed problem are static for $k \geq d + 1$.
Standard dynamic programming arguments allow us to first solve the Riccati equation for the time-invariant problem to get the positive definite solution $\tilde X_\star$ and the feedback gain $\tilde K_\star$, and then to solve the finite-horizon time-varying problem with
the cost function 
\begin{multline}
    J_i =\phixi[d]^\tran \tilde X_\star\phixi[d] + \sum_{k = 1}^d \Big( \phixi[k]^\tran \tilde Q[k]\phixi[k] +  \\
    2 v[k]^\tran \tilde Z\phixi[k] + v[k]^\tran \tilde R[k] v[k] \Big).
\end{multline}

The finite-horizon LQR problem has the solution for $k = 1, \ldots, d$:
\begin{multline}
        \tilde X[k] =\tilde Q[k] + \tilde A[k]^\tran \tilde X[k + 1] \tilde A[k]  \\ 
        - \left(\tilde A[k]^\tran \tilde X[k+1] \tilde B[k] + \tilde Z[k]\right) \left(\tilde R[k] + \tilde B[k]^\tran \tilde X[k + 1]B[k]\right)^{-1} \\
        \cdot \left(\tilde B[k]^\tran \tilde X[k + 1]\tilde A[k] \right),
\end{multline}
and
\begin{multline}
    \tilde K[k] = \left(\tilde R[k] + \tilde B[k]\tilde X[k + 1]\tilde B[k]\right)^{-1} \\
    \left(\tilde B[k]^\tran \tilde X[k + 1]\tilde A[k] + \tilde Z[k]^\tran \right).
\end{multline}

Finally, substituting $v_k = \tilde K[k]\phixi[k]$ into \onote{fix references} we get
\[
    \begin{aligned}
        \phixi[k + 1] & = (A + K[k])\phixi[k], \quad \phixi[1] = e_i \\
        \phiui[k] & = K[k]\phixi[k],
    \end{aligned}
\]
where 
\[
    K[k] = M_u[k]\left(F[k]^\dagger M_x[k + 1]A + F[k]N_F[k]\tilde K[k] \right)
\]

\section{Experiments}
\label{sec:simulation}


\section{CONCLUSIONS AND FUTURE WORKS}


==> tex_files/03_conclusions.tex <==
\subsection{Conclusions}
\subsection{Future Works}
